Wan-Animate-2: Pushing the Application Boundaries of Character Animation

Character image animation remains a foundational yet challenging task in computer vision. Existing approaches can be broadly categorized into three paradigms: methods based on explicit motion representations suffer from extraction errors and identity drift; methods based on implicit motion features lose fine-grained dynamics through compression; and in-context learning approaches avoid intermediate representations but incur prohibitive computational costs. Furthermore, all current systems are designed for offline synthesis, unable to meet the real-time requirements of interactive applications such as digital avatars and live-streaming hosts. To address these limitations, we present Wan-Animate-2, an end-to-end character animation framework that directly consumes the driving video within a redesigned Diffusion Transformer. Our architecture achieves superior motion fidelity and identity preservation by eliminating intermediate motion extractors entirely. We further introduce text driven viewpoint control that decouples the output camera perspective from the driving video--a capability rarely supported by prior character animation methods that rely on explicit motion representations. Beyond generation quality, we present Wan-Animate-2-Lite, an efficient variant that reduces inference latency to real-time thresholds through a three-stage training paradigm: teacher forcing pretraining with error buffer mechanism, and Self-Forcing distillation with chunk-wise backpropagation. This enables streaming character animation for interactive applications, opening new deployment scenarios that were previously infeasible. Qualitative evaluations and user studies demonstrate that Wan-Animate-2 achieves high-fidelity animation results across diverse characters and motion patterns. To foster further research and community development, we will release the Wan-Animate-2-Base model weights to the public.

==> figures/1_intro/radar_report.tex <==
% \begin{figure}[!ht]
%     \centering
%     \makebox[\linewidth][c]{%
%     \includegraphics[trim=7pt 7pt 7pt 7pt, clip, width=1.2\linewidth]{imgs/1_intro/advanced_comparison_paper.png}%
%   }
    
%     \caption{Comprehensive Human Evaluation across diverse generative tasks. We report a composite \textbf{Win Score} ($\frac{\text{Wins} + 0.5 \times \text{BothGood}}{\text{Total}}$) for Text-to-Image and General Editing, and \textbf{Pass Rate} for Interactive Editing and Series Generation.}
%     \label{fig:radar_report}
% \end{figure}

\begin{figure}[!hb]
    \centering
    \vspace{-2mm}
    \makebox[\linewidth][c]{%
    \includegraphics[width=0.78\linewidth]{imgs/1_intro/advanced_comparison.pdf}%
  }
    
    \caption{Comprehensive Human Evaluation across diverse generative tasks. We report a composite \textbf{Win Score} ($\frac{\text{Wins} + 0.5 \times \text{BothGood}}{\text{Total}}$) for Text-to-Image and General Editing, and \textbf{Pass Rate} for Interactive Editing and Series Generation.}
    \vspace{-20mm}
    \label{fig:radar_report}
\end{figure}

==> figures/1_intro/showcase_results.tex <==
\begin{figure}[!htb]
    \centering
    \vspace{-20pt}
    \makebox[\linewidth][c]{
        \includegraphics[width=1.1\linewidth]{imgs/1_intro/showcase_t2i.pdf}
    }
    \caption{Visual demonstration of diverse capabilities in text-to-image generation.}
    \label{fig:showcase_t2i}
\end{figure}

\clearpage

\begin{figure}[!htb]
    \centering
    \vspace{-20pt}
    \makebox[\linewidth][c]{
        \includegraphics[width=1.1\linewidth]{imgs/1_intro/showcase_i2i.pdf}
    }
    \caption{Visual demonstration of diverse capabilities in image-to-image generation (\eg, reference-based generation, instruction-based editing, and interactive editing).}
    \label{fig:showcase_i2i}
\end{figure}

\clearpage

\begin{figure}[!htb]
    \centering
    \vspace{-20pt}
    \makebox[\linewidth][c]{
        \includegraphics[width=1.1\linewidth]{imgs/1_intro/showcase_t2s.pdf}
    }
    \caption{Visual demonstration of diverse capabilities in image series generation.}
    \label{fig:showcase_t2s}
\end{figure}

\clearpage

\begin{figure}[!htb]
    \centering
    \vspace{-20pt}
    \makebox[\linewidth][c]{
        \includegraphics[width=1.1\linewidth]{imgs/1_intro/showcase_mix.pdf}
    }
    \caption{Visual demonstration of diverse capabilities in extreme aspect ratio adaptation, hyper-diverse realistic portrait generation, palette-guided generation, true alpha-channel generation, \etc.}
    \label{fig:showcase_mix}
\end{figure}

\begin{figure}[!htb]
    \centering
    \vspace{-20pt}
    \makebox[\linewidth][c]{
        \includegraphics[width=1.1\linewidth]{imgs/1_intro/showcase_t2i_more_1.pdf}
    }
    \caption{Visual demonstration of diverse capabilities in ultra-long text rendering.}
    \label{fig:showcase_t2i_more_1}
\end{figure}


\clearpage

==> figures/2_data/data_caption.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/2_data/data_caption.pdf}
    \caption{Overview of the structured data taxonomy. Our framework routes images into five primary categories and assigns them category-specific attributes (\eg, Lighting for photorealistic images, Axis for charts).}
    \label{fig:data_taxonomy}
\end{figure}

==> figures/2_data/data_distribution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{imgs/2_data/data_distribution_sunburst.png}
    \caption{Dataset category distribution (\%) for Text-to-Image, Image-to-Image, and Image Series.}
    \label{fig:data_distribution}
\end{figure}

==> figures/2_data/data_retrieval.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.75\linewidth]{imgs/2_data/data_retrieval.pdf}
    \caption{Overview of the multi-modal retrieval system.}
    \label{fig:data_retrieval}
\end{figure}

==> figures/2_data/data_understanding.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/2_data/understanding_data.pdf}
    \caption{Overview of the construction workflow for understanding data.}
    \label{fig:understanding_data}
\end{figure}

==> figures/2_data/filtering_operator.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{imgs/2_data/filtering_operator.pdf}
    \caption{Distribution and visual examples of the representative filtering operators.}
    \label{fig:filtering_operator}
\end{figure}

==> figures/3_model/model_framework.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/3_model/framework.pdf}
    \caption{
    Overview of the \wan architecture.
    }
    \label{fig:framework}
\end{figure}


==> figures/3_model/showcase_pe.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/3_model/showcase_pe.pdf}
    \caption{
    Visual comparison of different variants of our PE.
    }
    \label{fig:showcase_pe}
\end{figure}

==> figures/3_model/showcase_refine.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/3_model/showcase_refine.pdf}
    \caption{
    Visual comparison of the generated results without the refiner and with the refiner. In high-fidelity mode, the refiner only improves the low-level image details without any structural changes. While in repair mode, refiner will make more significant modifications, such as fixing text errors, eliminating artifacts, \etc.  }
    \label{fig:showcase_refine}
\end{figure}

==> figures/3_model/showcase_vae.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/3_model/showcase_vae.pdf}
    \caption{Visual comparison of different VAE models. Wan-Image VAE preserves clearer character-level details than existing methods.}
    \label{fig:vae_visual}
\end{figure}

==> figures/4_train/rl_framework.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/4_train/rl_framework.pdf}
    \caption{Overview of the reinforcement learning with human feedback framework (Left). Percentage improvement in Win Score of reinforcement learning over the SFT baseline (Right). }
    \label{fig:rl_framework}
\end{figure}




==> figures/4_train/showcase_distill.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/4_train/showcase_distill.pdf}
    \caption{
    Visual comparison of the results generated by the teacher model and the distilled student model.
    }
    \label{fig:distill}
\end{figure}

==> figures/4_train/showcase_rl.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/4_train/showcase_rl_t2i.pdf}
    \caption{
    Visual comparison of the results generated by the SFT base model and Cascade RL in T2I generation.
    }
    \label{fig:rl_case_t2i}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/4_train/showcase_rl_i2i.pdf}
    \caption{
    Visual comparison of the results generated by the SFT base model and Cascade RL in I2I generation.
    }
    \label{fig:rl_case_i2i}
\end{figure}

==> figures/5_eval/compare_visual.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/compare_t2i_i2i.pdf}
    \caption{Visual comparison with several models in T2I and I2I generation.}
    \label{fig:compare_t2i_i2i}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.87\textwidth]{imgs/5_eval/compare_ti2g.pdf}
    \caption{Visual comparison with several models in TI2S generation.}
    \label{fig:compare_ti2g}
\end{figure}

==> figures/5_eval/morecase_pe.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{imgs/5_eval/morecase_pe.pdf}
    \caption{
    Visual comparison of the results generated without the PE and with the PE.
    }
    \label{fig:morecase_pe}
\end{figure}

==> figures/5_eval/morecase_rl.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/5_eval/morecase_rl.pdf}
    \caption{
    Visual comparison of the results generated by the SFT base model and Cascade RL in T2I and I2I tasks.
    }
    \label{fig:rl_morecase}
\end{figure}

==> figures/5_eval/showcase_results_more.tex <==

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_t2i_more_2.pdf}
    \caption{More visual demonstration of diverse capabilities in T2I generation.}
    \label{fig:showcase_t2i_more_2}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_i2i_more_1.pdf}
    \caption{More visual demonstration of diverse capabilities in I2I generation.}
    \label{fig:showcase_i2i_more_1}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_i2i_more_2.pdf}
    \caption{More visual demonstration of diverse capabilities in the interactive editing generation.}
    \label{fig:showcase_i2i_more_2}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_t2s_more_1.pdf}
    \caption{More visual demonstration of diverse capabilities in T2S and TI2S generation.}
    \label{fig:showcase_t2s_more_1}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_t2s_more_2.pdf}
    \caption{More visual demonstration of diverse capabilities in T2S and TI2S generation.}
    \label{fig:showcase_t2s_more_2}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_mix_more_1.pdf}
    \caption{More visual demonstration of diverse capabilities in hyper-diverse realistic portrait generation, palette-guided generation, logical image series generation, \etc.}
    \label{fig:showcase_mix_more_1}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{imgs/5_eval/showcase_mix_more_2.pdf}
    \caption{More visual demonstration of diverse capabilities in logical image series generation, extreme aspect ratio adaptation, true alpha-channel generation, ultra-long text rendering, \etc.}
    \label{fig:showcase_mix_more_2}
\end{figure}


==> figures/5_eval/showcase_train_stage.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.92\textwidth]{imgs/5_eval/compare_train.pdf}
    \caption{Visual comparison of the generated results across different training stages.}
    \label{fig:showcase_train_stage}
\end{figure}

==> tables/training_details.tex <==
\begin{table}[t]
\centering
\small 
\caption{Detailed configurations for the training stages of both understanding and generation. U-CT, U\&M SFT, and OPD denote Understanding CT, Understanding \& Multi-task SFT, and On-Policy multi-teacher Distillation, respectively. PT, CT, and SFT denote Pre-training, Continual Pre-training, and Supervised Fine-tuning for the generation part.}
\setlength{\tabcolsep}{2pt} % Adjusting column spacing to fit 7 columns

\begin{tabularx}{\linewidth}{@{} l *{3}{>{\centering\arraybackslash}X} | *{3}{>{\centering\arraybackslash}X} @{}}
\toprule
 & \multicolumn{3}{c}{\textbf{Understanding}} & \multicolumn{3}{c}{\textbf{Generation}} \\
\textbf{Configuration} & \textbf{U-CT} & \textbf{U\&M SFT} & \textbf{OPD} & \textbf{PT} & \textbf{CT} & \textbf{SFT} \\
\midrule

\multicolumn{7}{@{} l}{\textit{\textbf{Training Process}}} \\ \addlinespace[2pt]
Steps (K)       & 46             & 10               & 0.4              & 713            & 223              & 13               \\
Tokens (T)      & 0.1            & 0.033            & 0.0016           & 13.27          & 8.85             & 0.62             \\
Resolution      & -              & -                & -                & 192/320/640        & 512-2048         & 512-2048         \\
Batch Size (K)  & 1              & 1.6              & 0.256            & 50/23/12       & 5                & 4                \\
\midrule

\multicolumn{7}{@{} l}{\textit{\textbf{Data Distribution}}} \\ \addlinespace[2pt]
Type            & T2T/I2T      & Multi-task*      & -                & T2I/I2I      & \multicolumn{2}{c}{T2I/I2I/T2S/TI2S} \\
Ratio           & 2:7          & 1:1:2:2:4        & -                & 7:3          & \multicolumn{2}{c}{7:2:0.5:0.5} \\
\midrule

\multicolumn{7}{@{} l}{\textit{\textbf{Hyperparameters}}} \\ \addlinespace[2pt]
Optimizer       & AdamW          & AdamW            & AdamW            & \multicolumn{3}{c}{AdamW} \\
Weight Decay    & 0.05           & 0.1              & 0.01             & \multicolumn{3}{c}{0.02} \\
Grad. Norm Clip & 1.0              & 1.0              & 0.2                & \multicolumn{3}{c}{0.5} \\
Uncond. Dropout & -              & -                & -                & \multicolumn{3}{c}{0.05} \\
Learning Rate   & $1 \times 10^{-5}$ & $7 \times 10^{-6}$ & $1 \times 10^{-6}$ & $5 \times 10^{-5}$ & $5 \times 10^{-5}$ & $3 \times 10^{-5}$ \\
EMA Ratio       & -              & 0.9998           & -                & 0.9999         & 0.9999           & 0.9998           \\
\bottomrule
\multicolumn{7}{l}{\scriptsize * Multi-task: T2T / I2T / T2I / I2I / Interleaved generation}
\end{tabularx}
\label{tab:training_details}
\end{table}

==> tables/understanding_results.tex <==
\begin{table}[htbp]
\centering
\caption{
Comparison of model performance on representative understanding metrics. ``--'' indicates that the indicator is missing in the relevant report.}

\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llccccccccccccc}
\toprule
 & & \multicolumn{8}{c}{Image Understanding} & \multicolumn{5}{c}{Text Understanding} \\
\cmidrule(lr){3-10} \cmidrule(lr){11-15}
Type & Model & \rot{MMMU} & \rot{MMStar} & \rot{MathVista} & \rot{HalluBench} & \rot{MMBench} & \rot{OCRBench} & \rot{AI2D} & \rot{Avg.} &\rot{AIME2025} & \rot{GPQA} & \rot{HLE} & \rot{LCBV6} & \rot{Avg.}\\
\midrule
\multirow{7}{*}{Und. Only} 
 & Qwen2-VL-7B & 54.1 & 60.7 & 58.2 & 50.6 & 80.7 & 86.6 & 83.0 & 67.7& -- & 30.3 & 2.8 & 9.7 &10.7\\
 & Qwen2.5-VL-7B & 58.6 & 63.9 & 68.2 & 52.9 & 82.6 & 86.4 & 83.9 &70.9 & -- & 34.3 & 2.7 & 14.9 & 13.0\\
 & Ovis2-8B & 57.4 & 64.6 & 71.8 & 56.3 & 83.6 & 89.1 & 86.6 &72.8 & -- & 35.9 & 4.2 & 20.0 & 15.0\\
 & InternVL3-8B & 62.7 & 68.2 & 71.6 & 49.9 & 81.7 & 88.0 & 85.2 &72.5& -- & 36.4 & 4.4 & 16.5 & 14.3\\
 & InternVL2.5-8B & 56.2 & 62.8 & 64.5 & 50.1 & 83.2 & 82.2 & 84.5 &69.1& 3.3 & 28.3 & 3.3 & 10.3 & 11.3\\
 & Kimi-VL-2506 (Thinking) & 64.0 & 70.4 & 80.1 & 59.8 & 84.4 & 86.9 & 81.9 &75.4& 33.3 & 45.5 & 2.3 & 29.7 & 27.7\\
\midrule
\multirow{8}{*}{Unified} 
 & BAGEL-7B & 55.3 & -- & 73.1 & -- & 85.0 & -- & -- & -- & -- & -- &-- & -- &--\\
 & UniWorld-V1 & 58.6 & -- & -- & -- & 83.5 & -- & -- & -- & -- & -- &-- & -- &--\\
 & MUSE-VL & 50.1 & -- & 55.9 & -- & 81.8 & -- & -- & -- & -- & -- &-- & --& --\\
 & Emu3 & 31.6 & -- & -- & -- & 58.5 & 68.7 & 70.0 & -- & -- & -- &-- & -- &--\\
 & MetaMorph & 41.8 & -- & -- & -- & 75.2 & -- & -- & -- & -- & -- &-- & -- &--\\
 & Janus-Pro-7B & 41.0 & -- & -- & -- & 79.2 & -- & -- & -- & -- &-- & -- & -- &--\\
 & BLIP3-o 8B & 50.6 & -- & -- & -- & 83.5 & -- & -- & -- & -- &-- & -- & -- &--\\
 \rowcolor{Gray}
 & Ours Instruct & 58.0 & 68.0 & 73.5 & 55.4 & 82.7 & 84.8 & 85.1 &72.5& 30.0 & 44.8 & 3.4 & 32.6 &27.7\\
 \rowcolor{Gray}
 & Ours Thinking & 67.4 & 72.8 & 82.3 & 57.7 & 83.5 & 84.1 & 86.1 &76.3& 33.3 & 47.0 & 3.9 & 31.4 &28.9\\
\bottomrule
\end{tabular}
\label{tab:understanding_results}
\end{table}

==> tables/vae_tab1.tex <==
\begin{table}[t]
\centering
\caption{Reconstruction comparison on 5,000 RGB images at 512p resolution. The best results are in \textbf{bold}.}
\label{tab:rgb_recon}
\setlength{\tabcolsep}{9pt}
\begin{tabular}{lccccc}
\toprule
Method & Spatial Downsampling & Latent Dim. & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
FLUX.1 VAE              & $8\times8$   & 16 & 34.769 & \textbf{0.958} & \textbf{0.009} \\
SD3.5 VAE            & $8\times8$   & 16 & 33.000 & 0.942          & 0.012 \\
Qwen-Image-Layered VAE         & $8\times8$   & 16 & 33.447 & 0.946          & 0.020 \\
HunyuanImage-3.0 VAE & $16\times16$ & 32 & 33.735 & 0.939          & 0.022 \\
Wan2.2 VAE           & $16\times16$ & 48 & 33.708 & 0.946          & 0.014 \\
\rowcolor{Gray}
\textbf{Wan-Image VAE} & $16\times16$ & 48 & \textbf{35.429} & \textbf{0.958} & 0.010 \\
\bottomrule
\end{tabular}
\label{tab:vae_1}
\end{table}

==> tables/vae_tab2.tex <==
\begin{table}[t]
\centering
\caption{Reconstruction comparison on 500 RGBA images at 1080p resolution. The best results are in \textbf{bold}.}
\label{tab:rgba_recon}
\setlength{\tabcolsep}{9pt}
\begin{tabular}{lccccc}
\toprule
Method & Spatial Downsampling & Latent Dim. & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
AlphaVAE (FLUX.1)
& $8\times8$   & 16 & 36.797          & 0.970          & 0.035 \\
Qwen-Image-Layered VAE     & $8\times8$   & 16 & 37.884          & \textbf{0.971} & \textbf{0.018} \\
\rowcolor{Gray}
\textbf{Wan-Image VAE} & $16\times16$ & 48 & \textbf{38.274} & 0.970 & \textbf{0.018} \\
\bottomrule
\end{tabular}
\label{tab:vae_2}
\end{table}
